Goal Representations for Instruction Following: A Semi-Supervised Language Interface to Control

Our goal is for robots to follow natural language instructions like "put the towel next to the microwave." But getting large amounts of labeled data, i.e. data that contains demonstrations of tasks labeled with the language instruction, is prohibitive. In contrast, obtaining policies that respond to image goals is much easier, because any autonomous trial or demonstration can be labeled in hindsight with its final state as the goal. In this work, we contribute a method that taps into joint image- and goal- conditioned policies with language using only a small amount of language data. Prior work has made progress on this using vision-language models or by jointly training language-goal-conditioned policies, but so far neither method has scaled effectively to real-world robot tasks without significant human annotation. Our method achieves robust performance in the real world by learning an embedding from the labeled data that aligns language not to the goal image, but rather to the desired change between the start and goal images that the instruction corresponds to. We then train a policy on this embedding: the policy benefits from all the unlabeled data, but the aligned embedding provides an interface for language to steer the policy. We show instruction following across a variety of manipulation tasks in different scenes, with generalization to language instructions outside of the labeled data. Videos and code for our approach can be found on our website: https://rail-berkeley.github.io/grif/ .

==> backup-2-method.tex <==
\newcommand{\D}[0]{\mathcal{D}}
\section{Problem Setup}
\label{sec:approach}

\begin{figure}
	\centering
	\includegraphics[width=.95\linewidth]{images/datasplits-new.png}
	\caption{Example trajectories within the Bridge Dataset. There are 47k trajectories in $\DB$ and 7k in $\DA$, but only those in $\DA$ have language annotations.}
	\label{fig:bridge}
\end{figure}

Our objective is to train robots to solve tasks specified by natural language instructions through interactions with the environment. 
This problem can be formulated by a conditional Markov Decision Process (MDP) denoted by the tuple $(\mathcal{S},\mathcal{A}, \rho, P, \mathcal{W}, \gamma)$ with state space $\mathcal{S}$, action space $\mathcal{A}$, initial state probability $\rho$, transition probability $P$, an instruction space $\mathcal{W}$, and discount factor $\gamma$. 
Each language-conditioned task can be defined by a pair of initial state $s_0 \in \mathcal{S}$ and an instruction $l \in \mathcal{W}$. 
Given the instruction $l$, the robot needs to take action $a_t \in \mathcal{A}$ at each time step $t$ to achieve success.
We assume that horizon $H$ is finite and the success conditioned is determined by the final state $s_H$ conditioned on $l$. 

To solve such tasks, we train a language-conditioned policy $\pi(a | s, l)$ on prior experiences collected and annotated by humans.
Since high-quality human annotations are expensive and time-consuming to obtain, we do not assume all the prior experiences to have labeled instructions. 
Instead, we assume the robot has access to a combination of two datasets -- a small-scale labeled dataset $\mathcal{D}_{A}$ with annotated instructions and a large-scale unlabeled dataset $\mathcal{D}_{B}$ consists of much more diverse play data collected in an open-ended manner.
Examples of these two datasets can be found in Figure~\ref{fig:bridge}.
The data is collected through teleoperation and the instructions are annotated through crowdsourcing.
We train $\pi(a | s, l)$ by imitating demonstration trajectories from both $\mathcal{D}_{A}$ and $\mathcal{D}_{B}$. 
We formulate $\pi(a | s, l)$ as a stochastic policy that predicts the Gaussian distribution $\mathcal{N}(\mu_a, \Sigma_a)$ where $\mu_a$ and $\Sigma_a$ are the means and standard deviation of the action $a$.
The policy $\pi(a | s, l)$ is trained through imitation learning, by maximizing the likelihood of the action $a$ sampled from the datasets. 








\section{\MethodName}

Our ultimate goal is to learn a language-conditioned policy $\pi(a | s, \ell)$. Approaches such as language-conditioned behavioral cloning (LCBC) directly learn this policy with a supervised loss on $\DA$ \cite{lynchInteractiveLanguageTalking2022}, but are unable to use the unannotated or autonomously collected data in $\DB$. Prior work has attempted to use both datasets by jointly training goal- and language-conditioned policies with a shared policy head: Learning from Play jointly trains $\pi(a | s, \ell)$ and $\pi(a | s, g)$, where the parameters of the policy head $\pi(a | s, \cdot)$ are shared \cite{lynchLanguageConditionedImitation2021}. Under the joint-training approach, representations of visual goals and instructions are implicitly aligned by the need to produce similar action plans. However, the goal representation is still free to encode information that is exclusive to visual goals. This limits the transfer of skills from unlabeled data as the jointly trained policy may learn to rely on spurious visual information that is absent when conditioned on language. 


We propose to explicitly align the representations of visual goals and language instructions. By mapping the representations to a shared space, we force the visual representations to abstract away spurious visual signals and focus on the semantic task, which is more robust to distractors, scene changes, and other forms of noise. Moreover, explicit alignment allows us to leverage existing resources that connect images and language. This includes vision-language models that have been pre-trained on millions of image-text pairs from cheap, non-robot settings (citation). 

We train our model in two stages. First, we use dataset $\DA$ to learn to map images and instructions to a shared task representation space. For initial state $s_0$, goal $g$, and instruction $ l$ from a trajectory in $\DA$, we train encoders $f_{\varphi}$ and $h_{\psi}$ with a contrastive objective such that $f_\varphi(\ell)$ and $h_\psi(s_0,g)$ are close for the same task and far away for distinct ones. We show that the naive CLIP-style approach of aligning $g$ and $l$ cannot adequately represent tasks, and describe a simple modification that allows us to leverage pretrained CLIP despite the different alignment objective. 

In the second stage, we train a single policy $\pi_\theta(a | s, \cdot)$ conditioned on representations from either modality. The language-conditioned policy is given by $\pi_\theta(a | s, f_\varphi(\ell))$, and the goal-conditioned policy by $\pi_\theta(a | s, h_\psi(s_0,g))$. We train them jointly on $\DA$ and train only the goal-conditioned policy on $\DB$ where $l$ is unavailable. The encoders can be optionally frozen or fine-tuned in this stage, both giving strong grounding and manipulation capabilities. 




\subsection{Learning Task Representations}

 



A pair $g, l$ from a trajectory in $\DA$ offers two different specifications of the same task -- one with a visual goal, and one with a language instruction. To align the two modalities, the naive approach may be to design an objective that draws the representations of $g$ and $l$ together. This is also the convenient choice, given that some vision-language models have already been pre-trained on similar objectives. For example, CLIP uses a contrastive InfoNCE objective to align image and text pairs, which past work has used to enable language-based navigation systems \cite{gadreCoWsPastureBaselines2022}. 

We argue, however, that the obvious choice of aligning $g$ and $l$ is inadequate to represent tasks in robotics. Goal images in tabletop manipulation, for example, can include the final state of multiple objects. The task itself is underspecified by the goal -- multiple courses of action could have lead to the same goal, and the goal representation must encode all such possibilities to be aligned with potential language instructions. 

Instead, we propose to reduce ambiguity in the task specification by introducing history through the initial state $s_0$. By comparing $g$ and $s_0$, it becomes possible for the encoder to attend to objects that are relevant to the task and leave out irrelavent ones. This vastly reduces the burden of the representations and can potentially improve robustness to distractors. Under this formulation, our task representations encode \textit{transitions} rather than goals. 

Concretely, our explicit alignment approach uses a contrastive InfoNCE objective \cite{oordRepresentationLearningContrastive2019} with a measure of cosine similarity $\cos(\cdot,\cdot)$ to align the visual task representation $h_\psi(s_0,g)$ and the language embedding $f_\varphi(\ell)$ on the dataset $\DA$. For simplicity, the following notation assumes that $\DA$ contains not full trajectories but $s_0, g, l$ tuples ($g^{(i)} = s_H^{(i)}$, where $H$ is the trajectory length). The objective can be written as: 
\def\x#1#2#3{#2_{#1}^{\ifx\relax#3\relax\else\scriptscriptstyle{(#3)}\fi}}
\def\1{\makebox[0pt][c]{\parbox[c]{7em}{\centering\scriptsize repel language from negative goal examples}}}
\def\2{\makebox[0pt][c]{\parbox[c]{7em}{\centering\scriptsize repel goals from negative language}}}
\def\3{\makebox[0pt][c]{\parbox[c]{6em}{\centering\scriptsize attract aligned representations}}}
\begin{align}
    \mathcal C_{ij} &:= e^{\cos(f_\varphi(\x{}\ell {i}),h_\psi(\x0s{j},\x Hs{j}))}/\tau \nonumber\\[4pt]
    \mathcal L_{\text{task}} &= 
    	\raisebox{2.5ex}{\math\displaystyle\mathop{\mathbb E}_{\substack{
    				\x0s{j_1}, \x Hs{j_1},\x{}\ell {j_1}\sim\DA\\
    				\ldots
    				\\[2pt] \x0s{j_k}, \x Hs{j_k},\x{}\ell {j_k}\sim\DA
    			}}\endmath}
    		\qty\Bigg[
    		\sum_{i=1}^k
    		 \underbrace{\log(\sum_{i'=1}^k \mathcal C_{j_ij_{i'}})}_{\1}
                + \underbrace{\log(\sum_{i'=1}^k \mathcal C_{j_{i'}j_{i}})}_{\2} 
                - \underbrace{\log{\mathcal C^2_{j_ij_i}}}_{\3}
    		~\;].
    \label{eq:task_loss}
\end{align}

We then tune
the policy network $\pi_\theta$ on top of these task representations with a behavioral cloning objective:
\begin{align}
    \mathcal L_{\text{policy}} =& 
    	-\frac{n_A}{n_A+n_B}\mathop{\mathbb E}_{s_0,s_i,a_i,s_{i+k},\ell\sim\DA} 
    	&& \kern -1em \log\pi_\theta(a_i |  s_i,f_\varphi(\ell))+\log \pi_\theta(a_i |  s,h_\psi(s_0,s_{i+k}))
   \nonumber\\
    &-\frac{n_B}{n_A+n_B}\mathop{\mathbb E}_{s_0,s_i,a_i,s_{i+k}\sim\DB} 
    && \kern -1em \log\pi_\theta(a_i |  s_i,h_\psi(s_0,s_{i+k})).
     \label{eq:policy_loss}
\end{align}

After learning representations, our final language-conditioned policy is $$\pi(a |  s, \ell)=\pi_\theta(a |  s,f_\psi(s_0,\ell)).$$


\subsection{Using Pre-trained Vision-Language Knowledge}

Our infoNCE task alignment objective in \Cref{eq:task_loss} learns aligned vision-language representations representing changes in the visual scene state. CLIP is an existing model for image-language alignment trained with a similar infoNCE contrastive objective on large-scale internet data \cite{radford2021clip}. CLIP contains broad semantic knowledge but cannot be directly used in our setting since it connects static images to goals rather than scene changes. In ablation X, we show that naively applying CLIP to our dataset cannot learn useful task representations for learning language-conditioned policies (link to ablation here). 

To learn dynamic task representations while retaining the semantic knowledge of CLIP, we make a simple modification to CLIP's image encoder and use it to initialize a $f(s_0, g)$ encoder which accepts a pair of images. Specifically, we use the vit-base model. It uses a patch embedding layer to project 3-channel images into tokens for the transformer architecture. The embedding layer is linear and implemented as multiplication with a weight matrix. We clone these weights and concatenate them along the channel dimension, creating a model that can accept $s_0$ and $g$ after they are stacked. We also half all the weights in the embedding layer so that $f(x, x) = f_{\text{CLIP}}(x)$ from the original encoder.



\subsection{Implementation Details}

We use the CLIP architecture to initialize our task encoders along with a ResNet-34 policy network.





